Feedforward-Feedback wake redirection for wind farm control

This work presents a combined feedforward-feedback wake redirection framework for wind farm control. The FLORIS wake model, a control-oriented steady-state wake model is used to calculate optimal yaw angles for a given wind farm layout and atmospheric condition. The optimal yaw angles, which maximize the total power output, are applied to the wind farm. Further, the lidar-based closed-loop wake redirection concept is used to realize a local feedback on turbine level. The wake center is estimated from lidar measurements \unit[3]{D} downwind of the wind turbines. The dynamical feedback controllers support the feedforward controller and reject disturbances and adapt to model uncertainties. Altogether, the total framework is presented and applied to a nine turbine wind farm test case. In a high fidelity simulation study the concept shows promising results and an increase in total energy production compared to the baseline case and the feedforward-only case.

==> images/tikzdefinitions.tex <==
\usepackage{tikz,pgfplots}%
\usetikzlibrary{shapes}%
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{calc}
\makeatletter \def\pgfplotscolormappdfmax{1} \def\pgfplotscolormappdfmax@inv{1000}
\usepackage{tikz-3dplot}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{positioning}
\usetikzlibrary{tikzmark}
\usetikzlibrary{arrows,shapes}
\usepgfplotslibrary{colorbrewer} 
\usetikzlibrary{pgfplots.colorbrewer}
\usepgfplotslibrary{patchplots}
\pgfplotsset{plot coordinates/math parser=false}%
\pgfplotsset{/pgf/number format/set thousands separator = {}}
\pgfplotsset{/pgf/number format/.cd,fixed,precision=4}%
\pgfplotsset{scaled ticks=false}%
\pgfplotsset{xticklabel shift={.05cm}}%
\pgfplotsset{yticklabel shift={.05cm}}%
\pgfplotsset{ylabel style={text width=3em,align=right}}%



\usepackage{calc}

 
 % my styles
\tikzstyle{MyNode2} = [draw=ColorLight, fill=ColorLight, rectangle, 
minimum height=4em, minimum width=2.5cm,rounded corners=1mm,inner sep=2mm,font=\normalsize\sffamily]

\tikzstyle{sum} = [draw=ColorDark, fill=ColorDark, circle,
node distance=\distance mm]

\tikzstyle{EstimationNode} = [draw=ColorLight, fill=ColorLight, rectangle, 
minimum height=4em, minimum width=2.5cm,rounded corners=1mm,inner sep=2mm,text=white,font=\normalsize\sffamily]

\tikzstyle{ControllerNode} = [draw=ColorC1, fill=ColorC1, rectangle, 
minimum height=4em, minimum width=2.5cm,rounded corners=1mm,inner sep=2mm,text=white,font=\normalsize\sffamily]

\tikzstyle{GeneralNode} = [draw=Color, fill=Color, rectangle, 
minimum height=4em, minimum width=2.5cm,rounded corners=1mm,inner sep=2mm,text=white,font=\normalsize\sffamily]

\tikzstyle{MiscNode} = [draw=ColorC2!50, fill=ColorC2!50, rectangle, 
minimum height=4em, minimum width=2.5cm,rounded corners=1mm,inner sep=2mm,text=black,font=\normalsize\sffamily]


